Unsupervised Learning with Stein's Unbiased Risk Estimator

Learning from unlabeled and noisy data is one of the grand challenges of machine learning. As such, it has seen a flurry of research with new ideas proposed continuously. In this work, we revisit a classical idea: Stein's Unbiased Risk Estimator (SURE). We show that, in the context of image recovery, SURE and its generalizations can be used to train convolutional neural networks (CNNs) for a range of image denoising and recovery problems without any ground truth data. Specifically, our goal is to reconstruct an image $x$ from a noisy linear transformation (measurement) of the image. We consider two scenarios: one where no additional data is available and one where we have measurements of other images that are drawn from the same noisy distribution as $x$, but have no access to the clean images. Such is the case, for instance, in the context of medical imaging, microscopy, and astronomy, where noise-less ground truth data is rarely available. We show that in this situation, SURE can be used to estimate the mean-squared-error loss associated with an estimate of $x$. Using this estimate of the loss, we train networks to perform denoising and compressed sensing recovery. In addition, we also use the SURE framework to partially explain and improve upon an intriguing results presented by Ulyanov et al. in "Deep Image Prior": that a network initialized with random weights and fit to a single noisy image can effectively denoise that image. Public implementations of the networks and methods described in this paper can be found at https://github.com/ricedsp/D-AMP_Toolbox.

==> Setup.tex <==
\section{Experimental Setup}\label{sec:Setup}

\rhcomment{I think this section disturbs the flow - why can't we mention this as we go; i.e., in the respective section explain the experiment in detail?
Happy to reorganize if ok for you.
}
\textcolor{red}{I think you're right. Please take a wack at it. I'm going to head back to Rice to start assembling the final data.}


Before describing our contribution, we first review the datasets, software, and network architectures that will be used in the experiments.

% In this work we conduct three sets of experiments, presented in Sections \ref{sec:Denoising}, \ref{sec:CS}, and \ref{sec:OneShotDenoising}. Here 
%Here we describe the datasets and software used in the experiments.%, which are presented in Sections \ref{sec:Denoising}, \ref{sec:CS}, and \ref{sec:OneShotDenoising}.


\begin{figure}[t]
\centering
\subfigure[]{\includegraphics[width=.16\textwidth]{figs/Gray_2092.png}}
\subfigure[]{\includegraphics[width=.16\textwidth]{figs/Gray_23025.png}}
\subfigure[]{\includegraphics[width=.16\textwidth]{figs/Gray_35010.png}}
\subfigure[]{\includegraphics[width=.16\textwidth]{figs/Gray_48055.png}}
\subfigure[]{\includegraphics[width=.16\textwidth]{figs/Gray_65132.png}}
\subfigure[]{\includegraphics[width=.16\textwidth]{figs/Gray_94079.png}}
\caption{6 representative training images from the BSD dataset.}\label{fig:TrainingImages}
%\end{figure}

%\begin{figure}[t]
%\centering
\subfigure[Barbara]{\includegraphics[width=.16\textwidth]{figs/barbara.png}}
\subfigure[Boat]{\includegraphics[width=.16\textwidth]{figs/boat.png}}
\subfigure[Couple]{\includegraphics[width=.16\textwidth]{figs/couple.png}}
\subfigure[House]{\includegraphics[width=.16\textwidth]{figs/house.png}}
\subfigure[Mandrill]{\includegraphics[width=.16\textwidth]{figs/mandrill.png}}
\subfigure[Bridge]{\includegraphics[width=.16\textwidth]{figs/streamandbridge.png}}
\caption{The 6 test images. They follow as similar distribution as the training images.} \label{fig:NaturalTestImages}
%\end{figure}

% %\begin{figure}[t]
% %\centering
% \subfigure[Flinstones]{\includegraphics[width=.16\textwidth]{figs/flinstones.png}}
% \subfigure[Fingerprint]{\includegraphics[width=.16\textwidth]{figs/fingerprint.png}}
% \subfigure[Yeast]{\includegraphics[width=.16\textwidth]{figs/Yeast.png}}
% \subfigure[Ecoli]{\includegraphics[width=.16\textwidth]{figs/Ecoli.png}}
% \subfigure[Rice Owl]{\includegraphics[width=.16\textwidth]{figs/RiceOwlSquareGray.png}}
% \subfigure[Pillars of Creation]{\includegraphics[width=.16\textwidth]{figs/PillarsofCreationSquareGray.png}}
% \caption{The 6 ``unnatural'' test images. They follow a different distribution than the training images.}\label{fig:UnnaturalTestImages}

\end{figure}

\paragraph{Dataset.}
Training images were pulled from Berkeley's BSD-500 dataset \cite{BSDDataset}. Example images are presented in Figure \ref{fig:TrainingImages}. 
%From this dataset, we used 400 images for training and 50 for validation. 
The training images were cropped, rescaled, flipped, and rotated to form a set of 204\,800 overlapping $40\times 40$ patches.% The validation images were cropped to form 10\,000 non-overlapping $40\times 40$ patches. 
We tested the methods on 6 standard test images presented in Figure \ref{fig:NaturalTestImages}.%, and a set of ``unnatural'' images presented in Figure \ref{fig:UnnaturalTestImages}. Unless otherwise noted, the networks were tested using $256\times 256$ versions of the test images.

\subsection{DnCNN}
The DnCNN image denoiser \cite{DnCNN} consists of 16 sequential $3\times 3$ convolutional layers with $64$ features at each layer. Sandwiched between these layers are ReLU and batch-normalization operations. DnCNN has a single skip connection to its output and is trained using residual learning \cite{residuallearning}.

\subsection{U-net}
U-net \cite{Unet} consists of a cascade $3\times 3$ convolution layers that are sequentially downsampled and then upsampled. Convolutional layers at each ``level'' of usampling/dowsampling are connected together by skip connections. The U-net we used had $128$ features at each convolution layer.

\paragraph{Implementation.}
The experiments in Sections \ref{sec:Denoising} and \ref{sec:CS} were performed using Tensorflow implementations of DnCNN \cite{DnCNN} and LDAMP \cite{LDAMP}. 
The experiments in Section \ref{sec:OneShotDenoising} were conducted using Torch implementations of U-net \cite{Unet} and MatConvnet implementations of DnCNN. 
The BM3D and CM3D \cite{BM3D} experiments were used Matlab implementations, based on compiled C. Public implementations of the algorithms can be found in the following locations:
\begin{itemize}
    \item DnCNN TensorFlow: \url{https://github.com/crisb-DUT/DnCNN-tensorflow}
    \item DnCNN MatConvnet: \url{https://github.com/cszn/DnCNN}
    \item LDAMP TensorFlow and MatConvnet: \url{https://github.com/cszn/DnCNN} 
    \item U-net Torch: \url{https://github.com/cszn/DnCNN}
    \item BM3D Matlab: \url{http://www.cs.tut.fi/~foi/GCF-BM3D/index.html#ref_software}
\end{itemize}



\paragraph{Training parameters.}
We trained all the networks using the Adam optimizer \cite{ADAMopt} with a training rate of 0.001. %., which we dropped to 0.0001 and then 0.00001 when the validation error stopped improving. 
We used mini-batches of 128 patches. The algorithms were trained and tested on a desktop with and Intel 6800K CPU and an Nvidia Pascal Titan X GPU.

\paragraph{Metrics.}
We report recovery accuracies in terms of PSNR, defined as 
\[
\text{PSNR}=10\log_{10}\bigg(\frac{255^2}{\|\hat{x}-x\|^2}\bigg),
\]
where all images lie in the range $[0,255]$.
Training and test times are provides in seconds.
%\paragraph{Hardware.}
%Training generally took between 3 and 5 hours per denoiser on an Nvidia Pascal Titan X.

% \paragraph{Testing setup.}
% We tested the algorithms with i.i.d.~Gaussian measurements and with measurements from a randomly sampled coded diffraction pattern \cite{candes2015phase}. The coded diffraction pattern forward operator was formed as a composition of three steps; randomly (uniformly) change the phase, take a 2D FFT, and then randomly (uniformly) subsample. 
% Except for the results in Figure \ref{fig:VisualComparo}, we tested the algorithms with $256\times 256$ images.# ($n=128^2$).
% We report recovery accuracy in terms of PSNR. We report run times in seconds. %This section summarizes the recovery results.

\paragraph{Propogating Gradients.}
Minimizing SURE requires propagating gradients with respect to the Monte Carlo estimate of the divergence \eqref{eqn:MCdiv_approx}. This is challenging to do by hand, but made easy but TensorFlow's auto differentiation capabilities.
